PEnG: Pose-Enhanced Geo-Localisation

Cross-view Geo-localisation is typically performed at a coarse granularity, because densely sampled satellite image patches overlap heavily. This heavy overlap would make disambiguating patches very challenging. However, by opting for sparsely sampled patches, prior work has placed an artificial upper bound on the localisation accuracy that is possible. Even a perfect oracle system cannot achieve accuracy greater than the average separation of the tiles. To solve this limitation, we propose combining cross-view geo-localisation and relative pose estimation to increase precision to a level practical for real-world application. We develop PEnG, a 2-stage system which first predicts the most likely edges from a city-scale graph representation upon which a query image lies. It then performs relative pose estimation within these edges to determine a precise position. PEnG presents the first technique to utilise both viewpoints available within cross-view geo-localisation datasets to enhance precision to a sub-metre level, with some examples achieving centimetre level accuracy. Our proposed ensemble achieves state-of-the-art precision - with relative Top-5m retrieval improvements on previous works of 213%. Decreasing the median euclidean distance error by 96.90% from the previous best of 734m down to 22.77m, when evaluating with 90 degree horizontal FOV images. Code will be made available: tavisshore.co.uk/PEnG

==> sections/peng_full.tex.tex <==
\begin{algorithm}
\caption{PEnG Algorithm}
\label{al:peng}
\begin{algorithmic}[1]
    \Require 
    Reference Primary Node Database $\eta^{sat}_{N}$,
    Query and Reference images $I^{street}_{Q}$ $I^{sat}_{R}$,
    Thresholds $\theta_{x} \in \{\theta_{pe}, \theta_{n},...\}$, 
    Reference Poses $\zeta_{r}^{E}$

    \Ensure $R_Q$
    
    \State \textbf{Stage 1 - CVGL}
    % Similarity scores from CVGL stage
    \For {$i = 1$ to $Q$}
        \State $\eta^{query}_{i} = \text{CNN}(I^{street}_{i})$
        \State $S_i = \text{scale}\biggl(\Bigl(\sum_{k}\eta^{ref}_{ik}\eta^{query}_{k}), 0, 1\Bigr)$
    \EndFor

    \State \textbf{Stage 2 - Pose}
    \State $i = 0, R = \text{array}_{Q}$
    \For {$j = 1$ to $Q$}
        % Until a threshold is met
        \While {$\text{thres}(R_{err}, \theta_{x})$} 
        
            % Filter node's edges by compass yaw
            $E_{cand} = \text{filter}(E(S_i), \Psi^j)$

            % Append query image and create exhaustive pairs
            $I^{pairs} = \textit{exhaustive}(E_{cand} + I_{i}^{street})$

            % Perform relative pose estimation
            $(R_j, t_j) = \text{RPE}(I^{pairs})$

            % Error to edge's avg rotation pose
            $R_{err} = \text{sim}_{euc}(R_j, \overline{E_{cand}})$

            $i = i + 1$
        \EndWhile
    \EndFor
    \State \Return Absolute Pose Estimations $R_Q$


\end{algorithmic}
\end{algorithm}

==> sections/ransacpnp.tex <==

\begin{algorithm}
\caption{Relative Pose Estimation Algorithm}\label{alg:ransac_pnp}
\label{al:ransacpnp}
\begin{algorithmic}[1]
\Require Set of 2D-3D corrs $\{ (x^i, X^i) \}_{i=1}^{N}$, number of iterations $k$, threshold $\epsilon$, minimum inliers $m$
, correspondences $p_{c}^{i}$, no. inliers $\iota^{i}$
\Ensure Estimated Relative Pose $\zeta =(R, t)$
\State Init \textit{best pose} and \textit{best no. inliers}
\For {$i = 1$ to $k$}
    \State Randomly sample 4 $p_{c}^{i}$ from $\{ (x_i, X_i) \}$
    \State Estimate pose $(R_i, t_i)$ using PnP on the sampled $p_{c}^{i}$
    \State Compute re-proj error for all points using $(R_i, t_i)$
    \State Select inliers with re-projection error $< \epsilon$
    \If {$\iota^{i}$ $> m$ \textbf{and} $\iota^{i}$ $>$ best no. inliers}
        \State Update best pose as $(R_i, t_i)$
        \State Update best no. inliers
    \EndIf
\EndFor
\State \Return best pose $\zeta$
\end{algorithmic}
\end{algorithm}
